Opportunities for Price Manipulation by Aggregators in Electricity Markets

Aggregators are playing an increasingly crucial role in the integration of renewable generation in power systems. However, the intermittent nature of renewable generation makes market interactions of aggregators difficult to monitor and regulate, raising concerns about potential market manipulation by aggregators. In this paper, we study this issue by quantifying the profit an aggregator can obtain through strategic curtailment of generation in an electricity market. We show that, while the problem of maximizing the benefit from curtailment is hard in general, efficient algorithms exist when the topology of the network is radial (acyclic). Further, we highlight that significant increases in profit are possible via strategic curtailment in practical settings.

==> tree_mesh_characterization.tex <==
\subsection{More General Congestions}
    \subsubsection{Results for tree network}
    While most of the transmission network contains cycles, there are proposals to extend the locational marginal pricing to distribution networks \cite{caramanis2012, sotkiewicz2006nodal, li2014} in order to properly incentivize distributed generation sources, and coordinating electric vehicle charging activities. Most of the distribution circuits are acyclic, in this case, we can simplify the analysis by the following lemma:
    \begin{lemma}
    In a tree network, nodes connected by uncongested lines have the same locational marginal price.
    \label{lemma: tree_simplify}
    \end{lemma}
By Lemma \ref{lemma: tree_simplify}, we can simplify the analysis of the whole network, to a reduced network that involves only the congested lines, and we can cluster the nodes connected by uncongested lines into one. 

Furthermore, the LMPs at a tree network have the following simple characterization
\begin{lemma}
In a tree network, nodes on the sending end of the congested line have equal or lower LMP compared to nodes at the receiving end. 
\label{lemma: tree_congestion}
\end{lemma}

Lemma \ref{lemma: tree_congestion} gives a heuristic that the aggregator has incentive to curtail generation to uncongest lines that has power flow to nodes with expensive generators; also, it will curtail so that the line between cheaper generator to the cluster that the aggregator is in is congested. 

\subsubsection{Results for mesh network}
%\niangjun{the following need to be verified ... }
\begin{lemma}
In a general network, node $i$ has equal or higher LMP than node $j$ if for all the congested lines, power flow in the same direction as the direction of flow induced by sending power from $j$ to $i$. 
\label{lemma: mesh_congestion}
\end{lemma}

\addtolength{\textheight}{-3cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.
